Personality, Culture, and System Factors - Impact on Affective Response to Multimedia

Whilst affective responses to various forms and genres of multimedia content have been well researched, precious few studies have investigated the combined impact that multimedia system parameters and human factors have on affect. Consequently, in this paper we explore the role that two primordial dimensions of human factors - personality and culture - in conjunction with system factors - frame rate, resolution, and bit rate - have on user affect and enjoyment of multimedia presentations. To this end, a two-site, cross-cultural study was undertaken, the results of which produced three predictve models. Personality and Culture traits were shown statistically to represent 5.6% of the variance in positive affect, 13.6% in negative affect and 9.3% in enjoyment. The correlation between affect and enjoyment, was significant. Predictive modeling incorporating human factors showed about 8%, 7% and 9% improvement in predicting positive affect, negative affect and enjoyment respectively when compared to models trained only on system factors. Results and analysis indicate the significant role played by human factors in influencing affect that users experience while watching multimedia.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

